Knowledge Completion for Generics using Guided Tensor Factorization

Given a knowledge base or KB containing (noisy) facts about common nouns or generics, such as "all trees produce oxygen" or "some animals live in forests", we consider the problem of inferring additional such facts at a precision similar to that of the starting KB. Such KBs capture general knowledge about the world, and are crucial for various applications such as question answering. Different from commonly studied named entity KBs such as Freebase, generics KBs involve quantification, have more complex underlying regularities, tend to be more incomplete, and violate the commonly used locally closed world assumption (LCWA). We show that existing KB completion methods struggle with this new task, and present the first approach that is successful. Our results demonstrate that external information, such as relation schemas and entity taxonomies, if used appropriately, can be a surprisingly powerful tool in this setting. First, our simple yet effective knowledge guided tensor factorization approach achieves state-of-the-art results on two generics KBs (80% precise) for science, doubling their size at 74%-86% precision. Second, our novel taxonomy guided, submodular, active learning method for collecting annotations about rare entities (e.g., oriole, a bird) is 6x more effective at inferring further new facts about them than multiple active learning baselines.

==> editted.tex <==
\input{AL}


%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation Methodology}

TODO: mention commonly used metrics for KBC and argue why they are not appropriate for the current task.

Reasoning in the science domain relies on high-precision facts. Accordingly, our goal for a tensor completion algorithm $A$ is to generate as many new true entries as possible at an acceptable precision level, e.g., 80\% precision. A natural metric for the task is therefore the \textbf{precision of $A$ at yield $y$}, defined as:
%
\begin{equation}
\prc_A(y) = \frac{1}{y} \sum_{i=1}^y v(t_i)
\end{equation}
%
where $t_1, \ldots, t_i$ denote the top scoring new entries predicted by $A$. This metric is, however, costly to evaluate exactly for large $y$, as it requires summing over the true values of all $y$ predictions. We describe below a method to obtain an $\alpha$-approximation of $\prc_A(y)$ for any $\alpha > 1$, using roughly only $\Delta \cdot \log_\alpha y$ queries for true values for some fixed constant $\Delta$. The method uses the notion of a $\Delta$-local variant of precision at a given yield, defined as follows:

\begin{definition}
\label{def:precision-at-yield}
Let $A$ be a tensor completion algorithm with predicting scoring function $s_A$. Let $t_1, t_2, \ldots, t_m$ be new tensor entries with non-increasing predicted scores, i.e., $s_A(t_i) \geq s_A(t_{i+1})$. Let $v(t_i)$ denote the true v of $t_i$, which is either $0$ (false) or $1$ (true). For $\Delta \in \mathbb{N}^+$, the \textbf{$\Delta$-precision of $A$ at yield $y$} is defined as:
\begin{equation}
\prc_A(y, \Delta) =
  \begin{cases}
    \frac{1}{y} \sum_{i=1}^y v(t_i) & \text{if\ } y < \Delta \\
    \frac{1}{\Delta} \sum_{i=y-\Delta+1}^y v(t_i) & \text{otherwise}
  \end{cases}
\end{equation}
\end{definition}

$\Delta$-precision may be viewed as a smoothed version of the true label sequence $v(t_1), v(t_2), \ldots, v(t_m)$. Although the actual label sequence, being a sequence of 0s and 1s, is erratic by design, we expect the density of 1s in this sequence to decrease with $t_i$ as $i$ increases. In other words, a sufficiently smoothed out variant of the label sequence should be non-increasing, except perhaps for the initial few values. This translates into $\prc_A(y, \Delta)$ being non-decreasing when $y$ and $\Delta$ are sufficiently large. We will use this monotonicity property to bound precision by functions of $\Delta$-precision.

We observe that $\prc_A(y)$ is simply $\prc_A(y, y)$. Further, when $y$ is a multiple of $\Delta$, $\prc_A(y)$ can be decomposed as $\frac{\Delta}{y} \sum_{j=1}^{y/\Delta} \prc_A(j \Delta, \Delta)$. Computing all of these uniformly spaced $y/\Delta$ local precision terms is, however, still as expensive as computing $\prc_A(y)$ directly. Following an idea used previously in a different context \cite{CITE-ICML-2013}, namely discrete integration for probabilistic graphical models, we instead \emph{approximately decompose} $\prc_A(y)$ using roughly only $\log_\alpha y$ local precision terms that are spaced based on a geometrically increasing spread with geometric ratio $\alpha$. We show that despite relying on logarithmically fewer queries, this method provides an $\alpha$-approximation of $\prc_A(y)$ for any $\alpha > 1$.

The geometrically spaced local precision terms are captured by the following expressions:

\begin{definition}
Let $\Delta, \ell, k \in \mathbb{N}^+$ and $\alpha > 1$. Define:
\begin{align}
L(\alpha, \ell, k, \Delta)
  & = \left \lfloor \frac{\alpha^\ell}{\Delta} \right \rfloor \prc_A(\alpha^\ell)
      + \sum_{j=\ell}^{k-1} \left \lfloor \frac{\alpha^j (\alpha - 1)}{\Delta} \right \rfloor \prc_A(\alpha^{j+1}, \Delta) \\
U(\alpha, \ell, k, \Delta)
  & = \left \lceil \frac{\alpha^\ell}{\Delta} \right \rceil \prc_A(\alpha^\ell)
      + \sum_{j=\ell}^{k-1} \left \lceil \frac{\alpha^j (\alpha - 1)}{\Delta} \right \rceil \prc_A(\alpha^j, \Delta)
\end{align}
\end{definition}

We show that if $\ell$ is chosen appropriately, then $L \leq U$, and $L$ and $U$ provide lower and upper bounds, resp., for $\prc_A$:
\begin{lemma}
\label{lem:sandwich}
Let $\Delta \in \mathbb{N}^+$ and $\alpha > 1$. Let $\tilde{y} \geq \Delta$ be such that $\prc_A(y, \Delta)$ is non-increasing for all $y \geq \tilde{y}$. Let $\ell = \lceil \log_\alpha \tilde{y} \rceil$. For all $k \geq \ell$:
\begin{equation}
\label{eqn:sandwich}
L(\alpha, \ell, k, \Delta) \leq \prc_A(\alpha^k) \leq U(\alpha, \ell, k, \Delta)
\end{equation}
\end{lemma}

\begin{proof}
TODO: add proof
\end{proof}

We next prove that $U$ is never more than $\alpha$ times $L$, thereby guaranteeing a good approximation:

\begin{lemma}
\label{lem:LU}
Let $\Delta, \ell, k \in \mathbb{N}^+$ and $\alpha > 1$. Then
\begin{equation}
\label{eqn:LU}
\alpha \cdot L(\alpha, \ell, k, \Delta) \geq U(\alpha, \ell, k, \Delta)
\end{equation}
\end{lemma}

\begin{proof}
TODO: address floors and ceiling properly!

To prove this result, we multiply both sides by $\Delta$ for convenience and apply a series of transformations:
%
\begin{align*}
\Delta \cdot \alpha \cdot L(\alpha, \ell, k, \Delta) \hspace{-12ex} \\
  & = \alpha^{\ell+1} \prc_A(\alpha^\ell) + \sum_{j=\ell}^{k-1} \alpha^{j+1}(\alpha - 1)\, \prc_A(\alpha^{j+1}, \Delta) \\
  & = \alpha^{\ell+1} \prc_A(\alpha^\ell) + \sum_{j=\ell+1}^k \alpha^j(\alpha - 1)\, \prc_A(\alpha^j, \Delta) \\
  & = \alpha^\ell \prc_A(\alpha^\ell) + \sum_{j=\ell}^k \alpha^j(\alpha - 1)\, \prc_A(\alpha^j, \Delta) \\
  & = \Delta \cdot U(\alpha, \ell, k, \Delta) + \alpha^k(\alpha-1)\, \prc_A(\alpha^k, \Delta) \\
  & \geq \Delta \cdot U(\alpha, \ell, k, \Delta)
\end{align*}
This concludes the proof.
\end{proof}

Combining the above two lemmas, we obtain:

\begin{theorem}
Let $A$ be a tensor completion algorithm, $\Delta \in \mathbb{N}^+$, $\alpha > 1$, and $\tilde{y} \geq \Delta$ be such that $\prc_A(y, \Delta)$ is non-increasing for all $y \geq \tilde{y}$. Let $\ell = \lceil \log_\alpha \tilde{y} \rceil$.
Then:
\begin{enumerate}
\item For any $k \geq \ell$, $L(\alpha, \ell, k, \Delta)$ and $U(\alpha, \ell, k, \Delta)$ are $\alpha$-approximations of $\prc_A(\alpha^k)$ from below and above, resp.

\item For any $y \geq \alpha^\ell$, let $k_- = \lfloor \log_\alpha y \rfloor$, and $k_+ = \lceil \log_\alpha y \rceil$. Then $L(\alpha, \ell, k_+, \Delta)$ and $U(\alpha, \ell, k_-, \Delta)$ are $\alpha^2$-approximations of $\prc_A(y)$ from below and above, resp.
\end{enumerate}
\end{theorem}

\begin{proof}
The $\alpha$-approximation result about $\prc_A(\alpha^k)$ follows immediately from Lemmas~\ref{lem:sandwich} and~\ref{lem:LU}.

For general $y \geq \alpha^\ell$, we consider the nearest exponents of $\alpha$ below and above $y$, which are $k_+$ and $k_-$. By the monotonicity of $\prc_A(y, \Delta)$ for all $y \geq \tilde{y}$, $\prc_A(y)$ is sandwiched between $\prc_A(\alpha^{k_+})$ and $\prc_A(\alpha^{k_-})$, which differ by at most a factor of $\alpha$ (TODO: EXPLAIN WHY!). Thus, $\prc_A(\alpha^{k_+})$ provides an $\alpha$-approximation of $\prc_A(y)$ from below. Since $L(\alpha, \ell, k_+, \Delta)$ provides a further $\alpha$-approximation of $\prc_A(\alpha^{k_+})$ from below, we obtain an $\alpha^2$-approximation as claimed. An analogous argument may be used to prove the claimed $\alpha^2$-approximation from above.
\end{proof}




==> notation.tex <==
\subsection{notation}
\hscomment{vector, matrix, norm, inner product, tensor, mode,  tensor decomposition, tensor rank, CP?, Tucker?}


